POSEIDON : Efficient Function Placement at the Edge using Deep Reinforcement Learning

Edge computing allows for reduced latency and operational costs compared to centralized cloud systems. In this context, serverless functions are emerging as a lightweight and effective paradigm for managing computational tasks on edge infrastructures. However, the placement of such functions in constrained edge nodes remains an open challenge. On one hand, it is key to minimize network delays and optimize resource consumption; on the other hand, decisions must be made in a timely manner due to the highly dynamic nature of edge environments. In this paper, we propose POSEIDON, a solution based on Deep Reinforcement Learning for the efficient placement of functions at the edge. POSEIDON leverages Proximal Policy Optimization (PPO) to place functions across a distributed network of nodes under highly dynamic workloads. A comprehensive empirical evaluation demonstrates that POSEIDON significantly reduces execution time, network delay, and resource consumption compared to state-of-the-art methods.

==> Figures/figure2.tex <==

\begin{figure}[t]
    \centering
    \begin{tikzpicture}[node distance=0.5cm, auto]

        % Pentagon coordinates
        \node (start) [process] at (90:4.5cm) {Simulate Various Payloads};
        \node (timesteps) [process] at (18:4.5cm) {Increase Number of Time-steps for Training};
        \node (training) [process] at (306:4.5cm) {Train RL Model};
        \node (deployment) [process] at (234:4.5cm) {Deploy on Edge Network};
        \node (monitoring) [process] at (162:4.5cm) {Monitor and Update Model};

        % Arrows
        \draw [arrow] (start) -- (timesteps);
        \draw [arrow] (timesteps) -- (training);
        \draw [arrow] (training) -- (deployment);
        \draw [arrow] (deployment) -- (monitoring);
        \draw [arrow] (monitoring) -- (start);

        % Initial arrow pointing to start node
        \draw [arrow] (6.5,4.5) -- (start)node[midway, above] {Deployment Life Cycle};

    \end{tikzpicture}
    \caption{The training and deployment process of the reinforcement learning model for an edge network. Initially, various payloads are simulated, and the number of timesteps for training is increased. The RL model is then trained and deployed on the edge network. Continuous monitoring and updating ensure the model adapts to local workload patterns.}
    \label{fig:rl_process}
\end{figure}

==> Tables/comparison.tex <==
% \begin{table}[ht]
% \centering
% \caption{Comparison of Neptune and Poseidon}
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Metric} & \multicolumn{2}{c|}{Poseidon} &\multicolumn{2}{c|}{Neptune} & \multicolumn{1}{c|}{CR-EUA} & \multicolumn{1}{c|}{VSVBP} \\
% \cline{2-5}
%  & $\alpha = 0$ & $\alpha = 1$ & $\alpha = 0$ & $\alpha = 1$ & & \\
% \hline
% Average Delay & 0 & 57.01 & 42.21 & 113.12 & 57.50 & 53.76 \\
% % \hline
% Average Cost & 251.67 & 50.33 & 95.63 & 50.33 & 84.2 & 84.80 \\
% % \hline
% Average Decision Time & 0.01 & 0.01 & 0.01 & 0.02 & 0.01 & 0.01 \\
% \hline
% \end{tabular}
% \label{tab:comparison}
% \end{table}



==> cuts.tex <==
% % \begin{itemize}
%     \todo[inline]{Introduce MEC}
%     \todo[inline]{Add a figure showing Agent overlooking / managing the community}
%     \todo[inline]{Please define what is a community as we are using it in the approach}

%     \red{Add this somewhere $\downarrow$\\
% Many real-world environments are inherently complex and dynamic, requiring flexible and adaptive learning methods. Deep RL's ability to handle non-linearities and complex interactions between states and actions makes it suitable for such environments.}

%     \red{Add this somewhere $\downarrow$\\
% Due to the high-dimensional nature of the placement problem and the continuous state space, it is impractical to use classical RL algorithms. As these algorithms typically rely on discrete state-action spaces, making it difficult to store and update values for each possible state-action pair in continuous spaces. Deep RL addresses this problem by using neural networks to approximate complex mappings from states to actions or action probabilities. This allows for more efficient and scalable representation and learning in high-dimensional state spaces.}
% % \end{itemize}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5 Original Overview
% \section{Approach Overview}
% \label{sec:approach}
% In this section, we present our approach for placing serverless functions at the edge, referred to as \approach. \approach leverages a combination of \textcolor{red}{deep reinforcement learning (remove this if abbreviated in intro)} \textcolor{green}{(Deep RL)} and  \textcolor{red}{Mixed Integer Programming} \textcolor{green}{MIP} to address the function placement and routing problem. The goal of the RL agent is to learn to place the functions in the community such that it minimizes both the (i) the overall network delay of the community, i.e the latency while serving function requests and (ii) the cost of running the function instances as well as ensuring a balance between these conflicting objectives with the help of a user defined trade-off to assign priorities to the same. The RL agent sequentially places functions using a state vector formed by using the relevant information from the community such as inter-node delays and available hardware resources as well as function parameters such as memory requirements. The workload of the function instance is also considered while making a placement decision, indicating the traffic of function requests at a particular node. This encoded information is used to infer an optimal function placement which satisfies our objectives \textcolor{red}{community}. \\
%  The function placement given by the agent is used to compute a routing policy for the community. To compute this routing policy, we utilize the generated function placements to formulate a MIP problem where the constraints are defined to handle the routing requests such that all function requests are redirected to only those nodes which have a running instance of the function. The objective of this problem is to minimize the network delay of the function requests and utilization of nodes, aligning with the objective of the agent.
% 
 % In this section, we present our approach for placing serverless functions at the edge, referred to as \approach. 
 % 
% \red{To compute the coefficients of request forwarding for each node-function-node triplet, we utilize the generated function placements to formulate a MIP problem. The constraints of this problem ensure that all function requests are redirected to nodes with a running instance of the function. The objective is to minimize the network delay of function requests and the utilization of nodes, aligning with the agent's objective. This problem formulation can then be solved (either optimally or pseudooptimally) via a prexisting solving strategy (such as COIN Branch and Cut \textit{solver} ).
%}
% 
% 
% 



% 
% \paragraph{Community} : Community is a collection of nodes that are situated geographically near each other.
% 
% \paragraph{Function Queue ($q_{func})$}: %
% Function queue contains all user requested function instances that needed to be deployed on the community. During sequential placement, this queue is updated after each successful placement and the placement episode ends when the function queue is empty.

% \paragraph{Static variables}: %
% $N$ represents the Number of nodes in the community. $F$ is used to represent the number of function instance requested on the community. $fn_{param}$ represnts the number of parameters used to represent function instance. $f_k$ refers to the current function in Function queue $q_{func}$  which is being placed.
% 
% 
% 
% \todo[inline]{Write the main approach and the mathematical formulation}
% 
% \todo[inline]{Write about function queue $q_{func}$}
% \todo[inline]{Explain how the agent works properly and mathematically}
% \todo[inline]{Explain the routing solver and the math and constraints behind it.}
% \todo[inline]{Use symbols to represent the info used to form the state vector and what each of those symbols mean}
% \todo[inline]{How is the reward calculated and rational behind it}
%\todo[inline]{Also whenever a new node is added the model needs to be retrained}
% \todo[inline]{The age}
% \todo[inline]{We haven't ordered the functions while placing them (If done to be added to overview)}



% Function instances whose user requests are received in the community require a running instance and hence, are considered for placement. These instances are placed in a function queue $q_{func}$ ordered by \red{???????? arrival time or heaviness}. %

% All functions deployment requests are collected at a community level and corresponding function instances are placed in the function queue, ordered by \red{???????? arrival time or heaviness}.

% \approach works in two phases iteratively for each function in the queue $q_{func}$.

% ########################### original start sec for poseidon placement phase
% For each function $f_i$ in the function queue $q_{func}$ \approach works in two phases%\red{iteratively}%
% . The first phase described in Section ~\ref{subsec:placement} is responsible for placing the function on the nodes it outputs a boolean row vector $\mathbf{c}$% 
% % \red{is responsible for calculating placement pattern on community}
% \red{use \textbf{c} here} and the second phase described in Section ~\ref{subsec:routing} is responsible is responsible for calculating the routing policy for a function $f_i$ among the nodes in the community according to the placement \red{pattern as} provided by phase 1 \red{maybe use the boolean vector \textbf{c} here}.
% ##################################################################3


% \approach works in two phases. Function instances whose user requests are received in the community require a running instance and hence, are considered for placement. All such function instances are placed in a function queue ordered by \red{???????}. For each function instance in the queue, the two phases occur sequentially. The sections ~\ref{subsec:placement} and ~\ref{subsec:routing} describe the two phases in detail.
% 
% 
% 
% such that for a given state $\mathcal{S}$ of the environment, $\pi(\mathcal{S}) \rightarrow \mathcal{A}$ where $\mathcal{A} \in \{0,1\}^N$ is the action space of the agent. The action space represents a set of boolean values corresponding to each node which denote whether the function instance needs to be placed on the node or not. The state $\mathcal{S}$ is a continuous state space consisting of information from the environment which affect the placement of the functions. Formally, $\mathcal{S}$ is a feature vector defined as:
% 

% 
% \footnote{Here, $\mathbf{X}'$ represents the flattened column vector of the matrix $\mathbf{X}$.}
% 
% Here, the constituent sub-matrices of the state vector are utilized as (i) $\mathbf{D}$ is required to \red{?????}, (ii) $\mathbf{A}$ is used to capture the available hardware resources at each node. This variable gets updated after placing each function instance to account for the resources consumed by the placed functions, (iii) Workload information $\mathbf{W}$ determines if a function needs to be placed on a specific node based on the amount of traffic on it, (iv) the function parameters $\mathbf{P}$, comprising CPU and \red{GPU?} memory requirements, alongside the mean and variance of CPU memory of remaining functions in the queue, guide placement decisions, (v) The total delay $\mathbf{T}$ assesses overall network delay post-function placement, guiding subsequent decisions to minimize system delay.

% \todo[inline]{Explain why Deep RL ? Not any classical algo like Q-Learning \downarrow}


% \approach leverages a combination of Deep Reinforcement Learning (Deep RL) and Mixed Integer Programming (MIP) to address the function placement and routing problem. The goal of \approach is to minimize both (i) the overall network delay of the community, i.e., the latency while serving function requests, and (ii) the cost of running the function instances while ensuring a balance between these conflicting objectives using a user-defined trade-off.
% %
% \approach first sequentially places functions using a state vector that incorporates relevant information from the community, such as inter-node delays, available hardware resources, and function parameters like memory requirements. The workload of the function instance, indicating the traffic of function requests at a particular node, is also considered. This encoded information is used to infer an optimal function placement by the Deep RL agent that satisfies our objectives.

% Then function placement determined by the agent is used to compute a routing policy for all requests of the function instance being processed. Every node $i$ in the community will have either an active function instance running or will route the request to another node $j$ with a running instance of that function. Even nodes with an active function instance can route a fraction of the total requests to other nodes in the community to manage their workload. To compute this routing policy, we utilize the generated function placements to formulate an Mixed Integer Programming problem. The constraints of this problem ensure that all function requests are redirected to nodes with a running instance of the function. The objective is to minimize the network delay of function requests and maximise the utilization of nodes, aligning with the agent's objective.
% % 
% \red{talk about state updation and reward calulation here}


% For each function $f_i$ in the function queue $q_{func}$, \approach works in two phases. The first phase, described in Section ~\ref{subsec:placement}, is responsible for placing the function on the nodes and outputs a boolean row vector $\mathbf{c}$. The second phase, described in Section ~\ref{subsec:routing}, is responsible for calculating the routing policy for a function $f_i$ among the nodes in the community according to the placement pattern provided by the boolean vector $\mathbf{c}$.


% \subsection*{Observation Space Components}

% 1. \textbf{Inter-Node Delays}:
% \[
% \mathbf{D} \in \mathbb{R}^{N \times N}
% \]
% where \(N\) is the number of nodes. Each element \(D_{ij}\) represents the network delay between node \(i\) and node \(j\).

% 2. \textbf{Available Resources}:
% \[
% \mathbf{A} \in \mathbb{R}^{N \times R}
% \]
% where \(N\) is the number of nodes and \(R\) is the number of resource features. Each element \(A_{ij}\) represents the availability of resource feature \(j\) on node \(i\).

% 3. \textbf{Function Workload}:
% \[
% \mathbf{W} \in \mathbb{R}^{N \times 1}
% \]
% where \(W_i\) represents the workload of the current function instance on node \(i\).

% 4. \textbf{Function Parameters}:
% \[
% \mathbf{P} \in \mathbb{R}^{1 \times F}
% \]
% where \(F\) is the number of function features. Each element \(P_{j}\) represents a parameter of the current function instance.

% 5. \textbf{Total Delay}:
% \[
% \mathbf{T} \in \mathbb{R}_{\geq 0}
% \]
% where \(\mathbf{T}\) is a scalar representing the total network delay of all the function instances that have been placed sequentially. The scalar is initialised with 0 while placing the first function in $q_{func}$ and is updated by adding the network delay incurred by placing the current function.

% 6. \textbf{Action Space}:

% The action space is represented as a multi-binary space, where each binary variable indicates whether a function is placed on a node.

% \[
% \mathbf{a} \in \{0, 1\}^{\text{N}}
% \]

% where \(\mathbf{a}_i = 1\) if the function is placed on node \(i\), and \(\mathbf{a}_i = 0\) otherwise.


% and incorporating the adaptive benefits of Deep RL techniques for placing functions on the edge. The RL agent is deployed on a community of nodes in a given network, it takes into consideration dynamic workloads and hardware resource constraints to calculate the optimal placement for function instances.

% \approach uses information from the community to form a state vector which is then used by the RL agent to decide the placements (which is a binary vector). Using this placement vector and then \approach uses an MIP formm

% % Oview of approach
% In this section, we present our proposed approach for function placement in edge computing called \approach. It leverages deep reinforcement learning system to address the function placement problem(formalize the problem in earlier sections) and to incorporate adaptive benefits of the deep learning technique into the problem for function placement on the edge. It deploys? an RL agent on a community of nodes in a given network considering dynamic workloads and hardware resources constraints in the community to calculate the placement for the function instances in the cluster in a sequential manner, also considering resources requested by the current function being placed as well as all other functions in the placement queue(q function?). \textcolor{red}{The function in the system are placed in order of their size calculated considering average workload and CPU and GPU memory requested}. This preprocessing allows for a more stable behaviour on introduction of new function instance on the network. The agent also considers other essential factors  such as inter node delays which allows it to learn the network behaviour and adapt to it. All considered parameters are passed as as feature vector to the agent \textcolor{red}{(show the break up diagram)}. \textcolor{red}{This also allows approach to model inactive nodes as dead nodes by passing available resources for those as null.}\textcolor{red}{(this line can be better framed)} The agent then uses deep reinforcement learning techniques to learn this behaviour. The approach also allows for a user defined RL technique as well as a trade-off factor that can be used to change learning behaviour of agent, providing a method to get trade-off between delay and cost for requested deployment.
% The Approach can be generalized to all deep rl techniques. In the following section we have explored techniques like PPO and \textcolor{red}{A2C ?} for testing and evaluation. The Inferred placement is then passed into a routing policy solver \textcolor{red}{based on optimization formulation \textbf{(need to elaborate)}}, which calculates the routing for the given placement under the constraints of minimizing delay using a MIP formulation.\textcolor{red}{(we can write about MIP?)} the calculated routing. The agent is also trained on the incoming data points to make the system adapt online with the environment. \textcolor{red}{(use Online learning)} This approach also has the benefit of reducing the overhead over other approaches such as modelling the entire problem as optimization problem or tackling the curse of dimensionality that arises in classical reinforcement learning formulations when dealing with large state space environments. The Approach also incorporates a metric recording system thus having the advantage of being easily extensible, incorporable and observable. 

% Mathematical modeling of approach: 
% (Algorithmic manner)

% $\text{Feature vector} = \text{environment param vector} \; || \; \text{Node param vector} \; \\|| \; \text{cur function param vector}  \;||\; \text{in q function vector ( a better word for in q sounds bad)}\; \\ ||\; \text{cur placement vector} || \text{network occupancy vector} \\\textcolor{red}{\text{Assign variable names to these vectors}}\uparrow$

% Environment Parameter Vector: $\mathbf{E}$\\
% Node Parameter Vector: $\mathbf{N}$\\
% Current Function Parameter Vector: $\mathbf{F_c}$\\
% In-Queue Function Vector: $\mathbf{Q}$\\
% Current Placement Vector: $\mathbf{P_c}$\\
% Network Occupancy Vector: $\mathbf{O}$


% Feature vector --> Agent --> Placement Vector ---> User
%                     ^           |
%             rewards |           |
%                     |           |
%             Environment <- - - -  - - - - -> Routing solver ---> Routing  policy

% Section wise detailing for the approach
% Nodes Modeling
% function Modelling
% Routing solver


% \begin{tikzpicture}[node distance=3cm, auto]

%     % Nodes
%     \node (feature) [draw, rectangle] {Feature vector};
%     \node (agent) [draw, rectangle, right of=feature] {Agent};
%     \node (placement) [draw, rectangle, right of=agent] {Placement Vector};
%     % \node (user) [draw, rectangle, right of=placement] {User};
%     \node (environment) [draw, rectangle, below of=agent, node distance=4cm] {Environment};
%     \node (solver) [draw, rectangle, right=of environment, xshift=1cm] {Routing solver};
%     \node (policy) [draw, rectangle, right of=solver] {Routing policy};

%     % Arrows
%     \draw[->] (feature) -- (agent);
%     \draw[->] (agent) -- (placement);
%     % \draw[->] (placement) -- (user);
%     \draw[->] (environment) -- (agent) node[midway, left] {rewards};
%     \draw[->] (environment) -- (solver);
%     \draw[->] (solver) -- (policy);
%     \draw[->] (solver) -- (environment);

%    % Arrow from Placement Vector to the arrow between Environment and Routing solver
%     \draw[-] (placement) -- ++(0,-4);

% \end{tikzpicture}







% \approach uses a feature extractor to extract a feature vector 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{itemize}
%      \item We're not ordering the functions
% \item We have a function queue which maintains all the function instances which need to be placed in the community.
% \item The RL agent starts an episode in which it sequentially picks up function instances to place in the community and inferences a placement for all instances sequentially.
% \begin{itemize}
    
% \item  For each inference , the procedure is composed of 
% 	\item Encoding the current state of the community and the compute requirements of the function instances along with the function workload, total network delay of tthe system at each step
% 	\item The model infers an boolean vector of size equal to the number of nodes currently in the community(not the upper bound on the number of nodes in the community, which implies that if the topology of the community is changed , the model needs to be retrained since number of nodes in the community are changed.This is because if the number of nodes passed compose of both active and dead nodes, the agent learns to place functions freely on the active nodes since the penalties for placing on entirely dead nodes tends to be much worse.) \todo[inline]{We can maybe put this in threats to validity?}
% 	\item This boolean vector is used to infer set of nodes to place the function instance on. The available compute resources of nodes on which the function is placed are then updated.
% 	\item The inferred placement is used to compute a routing policy using MIP with the objective to minimize network delay and cost by following a set of constraints(define the constraints).
% 	\item  The reward for the placement is calculated and used for training the agent(define reward model)
% \end{itemize}
% \item Write a small paragraph on PPO or whatever algorithm we are gonna use
% \item  Also write how our approach can be extended to more RL algorithms (like \textit{A2C}, \textit{PPO}, \textit{RecurrentPPO}, \textit{TRPO} \& \textit{Maskable PPO}) present in \textit{Stable Baselines 3}
% \end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\todo{Maybe bold the best results in each row?}

% \renewcommand{\arraystretch}{1.5}
% \begin{table}[ht]
% \centering
% \caption{Comparison of Poseidon with Other Approaches for Light Payload}
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Metric} & \multicolumn{2}{c|}{Poseidon} & \multicolumn{2}{c|}{Neptune} & \multicolumn{1}{c|}{\centering CR-EUA} & \multicolumn{1}{c|}{\centering VSVBP} \\
% \cline{2-5}
%  & $\alpha = 0$ & $\alpha = 1$ & $\alpha = 0$ & $\alpha = 1$ & & \\
% \hline
% Average Delay & 0 & 57.01 & 42.21 & 113.12 & 57.50 & 53.76 \\
% % \hline
% Average Cost & 251.67 & 50.33 & 95.63 & 50.33 & 84.2 & 84.80 \\
% % \hline
% Average Inference Time & 0.01 & 0.01 & 0.14 & 0.02 & 0.01 & 0.01 \\
% \hline
% \end{tabular}
% \label{tab:comparison_of_poseidon_and_neptune}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% VSVBP  when compared to VSVBP and CR-EUA. \approach is able to approximate solutions of a NP-Hard problem.

% the results are reported in the Tables ~\ref{tab:light:comparison_of_poseidon_and_neptune} and ~\ref{tab:heavy:comparison_of_poseidon_and_neptune} and Figures ~\ref{fig:light:eff_delay}, ~\ref{fig:light:eff_cost}, ~\ref{fig:heavy:eff_delay} and ~\ref{fig:heavy:eff_cost}.

% We can see from the table that \approach for $\alpha = 0$ the delay is $0$ this is because when $\alpha = 0$ the DRL agent only minimizes the delay as the cost is not considered a critical factor and the most optimal way to do that is to place the function on all nodes because of which the average cost is so high (251.67) this is expected as the DRL agent aims learn the most optimal policy. NEPTUNE has a higher average delay because it does not place a function on all the nodes even when $\alpha = 0$ and tries to minimize the disruptions as well. 

% We can also see from the Table ~\ref{tab:comparison_of_poseidon_and_neptune_heavy} that for $\alpha = 1$ (delay is not considered a critical factor here and only the cost is considered a critical factor) \approach performs better and has lower average delay than NEPTUNE. This can be attributed to the fact that \approach learns to place the functions near the to nodes where the request arrive and also route them through the shortest routes. CR-EUA has a higher cost than \approach as it tries to maximize the number of requests processed. Similarly VSVBP also has a higher cost than \approach as it tries to maximize the number of allocated user requests.

% When $\alpha = 0$ the DRL agent in \approach only places functions to minimize the cost. As a result, the delay is not considered as a critical factor, leading to an increase in delay. The cost reduction is achieved by choosing less expensive resources or routes, even if they are slower. When $\alpha = 1$ \approach only minimizes the delay. In this case, the system might select faster, albeit more expensive, resources or routes or even more nodes to reduce the workload on the overall topology, resulting in a decrease in delay but an increase in cost. \red{Whereas for NEPTUNE, MCF and CriticalityHeuristic, VSVBP for $\alpha = 0$ and $\alpha = 1$ the cost and delay are ?}

% ................
% ...................
% Figure \ref{} shows the plot representing the cost accrued by different approaches during the execution. As the plot demonstrates, \approach 

% @@@@Add a table of the evaluated metrics for Poseidon and Neptune to improve readability of the results.
% \todo[inline]{Observation -> At same alpha poseidon and neptune prioritize the objectives differently but POSEIDON achieves near optimal results. $\alpha = 1 \text{ means minimize cost } and \alpha = 0 \text{ means minimize delay}$}

% When $\alpha = 0$, we aim to minimize delay without considering cost, and when $\alpha = 1$, we aim to minimize cost without considering delay. However, when $\alpha = 0.5$, we seek a balance between minimizing both cost and delay. As shown in Figure~\ref{} and Figure~\ref{}, at $\alpha = 0.5$, the average delay for \approach is smaller than the average delay for NEPTUNE this is because Mixed Integer Programming is a NP-Hard problem whereas the cost \red{write about cost} for $\alpha = 1 \text{ or } \alpha = 0$ the average delay for \approach is greater than the average delay for NEPTUNE. The cost when \red{$\alpha = 1$ and $\alpha = 0$} for \approach is \red{?} whereas for NEPTUNE it is \red{}.

% As we can see from the \red{figure / table} ~\ref{} ~\ref{} when $\alpha = 0.5$ it means we're trying to balance the delay and cost the averarge delay for \approach is smaller than the average delay for NEPTUNE

==> instructions.tex <==
\begin{document}

\section{\textcolor{red}{Please write in the files in the Section folder}}
\section{\textcolor{red}{Please use main.tex}}
\textbf{Limit is 15 pages including, abstract figures and references.}
\subsection{A Subsection Sample}
Please note that the first paragraph of a section or subsection is
not indented. The first paragraph that follows a table, figure,
equation etc. does not need an indent, either.

Subsequent paragraphs, however, are indented.

\subsubsection{Sample Heading (Third Level)} Only two levels of
headings should be numbered. Lower level headings remain unnumbered;
they are formatted as run-in headings.

\paragraph{Sample Heading (Fourth Level)}
The contribution should contain no more than four levels of
headings. Table~\ref{tab1} gives a summary of all heading levels.

\begin{table}
\caption{Table captions should be placed above the
tables.}\label{tab1}
\begin{tabular}{|l|l|l|}
\hline
Heading level &  Example & Font size and style\\
\hline
Title (centered) &  {\Large\bfseries Lecture Notes} & 14 point, bold\\
1st-level heading &  {\large\bfseries 1 Introduction} & 12 point, bold\\
2nd-level heading & {\bfseries 2.1 Printing Area} & 10 point, bold\\
3rd-level heading & {\bfseries Run-in Heading in Bold.} Text follows & 10 point, bold\\
4th-level heading & {\itshape Lowest Level Heading.} Text follows & 10 point, italic\\
\hline
\end{tabular}
\end{table}


\noindent Displayed equations are centered and set on a separate
line.
\begin{equation}
x + y = z
\end{equation}
Please try to avoid rasterized images for line-art diagrams and
schemas. Whenever possible, use vector graphics instead (see
Fig.~\ref{fig1}).

\begin{figure}
\includegraphics[width=\textwidth]{fig1.eps}
\caption{A figure caption is always placed below the illustration.
Please note that short captions are centered, while long ones are
justified by the macro package automatically.} \label{fig1}
\end{figure}

\begin{theorem}
This is a sample theorem. The run-in heading is set in bold, while
the following text appears in italics. Definitions, lemmas,
propositions, and corollaries are styled the same way.
\end{theorem}
%
% the environments 'definition', 'lemma', 'proposition', 'corollary',
% 'remark', and 'example' are defined in the LLNCS documentclass as well.
%
\begin{proof}
Proofs, examples, and remarks have the initial word in italics,
while the following text appears in normal font.
\end{proof}
For citations of references, we prefer the use of square brackets
and consecutive numbers. Citations using labels or the author/year
convention are also acceptable. The following bibliography provides
a sample reference list with entries for journal
articles~\cite{ref_article1}, an LNCS chapter~\cite{ref_lncs1}, a
book~\cite{ref_book1}, proceedings without editors~\cite{ref_proc1},
and a homepage~\cite{ref_url1}. Multiple citations are grouped
\cite{ref_article1,ref_lncs1,ref_book1},
\cite{ref_article1,ref_book1,ref_proc1,ref_url1}.

\begin{credits}
\subsubsection{\ackname} A bold run-in heading in small font size at the end of the paper is
used for general acknowledgments, for example: This study was funded
by X (grant number Y).

\subsubsection{\discintname}
It is now necessary to declare any competing interests or to specifically
state that the authors have no competing interests. Please place the
statement with a bold run-in heading in small font size beneath the
(optional) acknowledgments\footnote{If EquinOCS, our proceedings submission
system, is used, then the disclaimer can be provided directly in the system.},
for example: The authors have no competing interests to declare that are
relevant to the content of this article. Or: Author A has received research
grants from Company W. Author B has received a speaker honorarium from
Company X and owns stock in Company Y. Author C is a member of committee Z.
\end{credits}

\end{document}
